Achieving robustness in classification using optimal transport with hinge regularization

Adversarial examples have pointed out Deep Neural Networks vulnerability to small local noise. It has been shown that constraining their Lipschitz constant should enhance robustness, but make them harder to learn with classical loss functions. We propose a new framework for binary classification, based on optimal transport, which integrates this Lipschitz constraint as a theoretical requirement. We propose to learn 1-Lipschitz networks using a new loss that is an hinge regularized version of the Kantorovich-Rubinstein dual formulation for the Wasserstein distance estimation. This loss function has a direct interpretation in terms of adversarial robustness together with certifiable robustness bound. We also prove that this hinge regularized version is still the dual formulation of an optimal transportation problem, and has a solution. We also establish several geometrical properties of this optimal solution, and extend the approach to multi-class problems. Experiments show that the proposed approach provides the expected guarantees in terms of robustness without any significant accuracy drop. The adversarial examples, on the proposed models, visibly and meaningfully change the input providing an explanation for the classification.

==> cvpr_parts/hkr_section.tex <==
%In this section we propose a regularized version of the Kantorovich-Rubinstein problem and we prove that it is still the dual of a transportation problem. Furthermore, we show that it has good properties in terms of robustness for classification problem.
\subsection{Definitions and primal transportation problem}
%\begin{figure}
%  \centering
%  \includegraphics[width=0.7\linewidth]{img/loss_function.png}
%  \caption{$\mathcal{L}_{\W pen}$ loss function with respect to $yf(x)$.}
%  \label{fig:loss}
%\end{figure}%
In order to improve the classification abilities of the classifier based on Wasserstein distance, we propose a Kantorovich-Rubinstein optimization problem regularized by an hinge loss :


\begin{equation} \label{eq:reg_OT} 
\begin{split} 
\sup_{f \in Lip_1(\Omega)}&-\mathcal{L}^{hKR}_\lambda(f) =\\ & \inf_{f \in Lip_1(\Omega)} \underset{\textbf{x} \sim P_-}{\mathbb{E}} \left[f(\textbf{x})\right]-\underset{\textbf{x} \sim P_+}{\mathbb{E}}\left[f(\textbf{x})\right] \\ &+\lambda\underset{\textbf{x}}{\mathbb{E}} \left(1-Yf(\textbf{x})\right)_+ \end{split} 
\end{equation}

where $(1-\textbf{y}f(\textbf{x}))_+$ stands for the hinge loss $max(0,1-\textbf{y}f(\textbf{x}))$ and $\lambda>=0$. We name $\mathcal{L}^{hKR}_\lambda$ the hinge-KR loss. The goal is then to minimize this loss with an 1-Lipschitz neural network.
When $\lambda=0$, this corresponds to the Kantorovich-Rubinstein dual optimization problem. Intuitively, the 1-Lipschitz function $f^*$ optimal with respect to Eq.~\eqref{eq:reg_OT} is the one that both separates the examples with a margin and spreads as much as possible the image of the distributions. When using only an hinge loss (as in \cite{li2019preventing} for instance), the examples outside the margin are no more taken into consideration. If the margin is increased to cover all the examples and if the class are equally distributed, the hinge loss becomes equivalent to the Kantorovich Rubinstein loss and then leads to a weak classifier. 

In the following, we introduce Theorems that prove the existence of such an optimal function $f^*$ and important properties of this function. Demonstrations of these theorems are in Appendix~\ref{appendix:proofs}.
\begin{Theorem} [Solution existence]
\label{Lemma:bounded_M}
 For each $\lambda>0$ there exists at least a solution $f^*$ to the problem  \[ f^*:=f_{\lambda}^*\in{\arg\min}_{f\in \text{Lip}_1(\Omega)}\mathcal{L}^{hKR}_{\lambda}(f) . \]
\end{Theorem}
Moreover, let $\psi$ be an optimal transport potential for the transport problem from $P_+$ to $ P_-$, $f^*$ satisfies that 
\begin{align}\label{eq:M}
	|| f^*||_{\infty}\leq M:= 1+\text{diam}(\Omega)+\frac{L_1(\psi)}{\inf(p,1-p)}.
\end{align}
%\footnote {{\color{red} (Franck) ne faudrait-il pas commenter l'apport de cette inégalité?  ?}}
The next theorem establishes that the Kantorovich-Rubinstein optimization problem with hinge regularization is still a transportation problem with relaxed constraints on the joint measure (which is no longer a joint probability measure).
\begin{Theorem}[Duality]\label{Theo:dual}
Set  $P_+, P_-\in \mathcal{P}(\Omega)$ and $\lambda>0$, then the following equality holds
\begin{align}\label{eq:dual}
\begin{split}
 \sup_{f\in \text{Lip}_1(\Omega)}- \mathcal{L}^{hKR}_\lambda(f)=&	\inf_{\pi \in\Pi^p_{\lambda}(P_+, P_-)}\int_{\Omega\times \Omega}|{\textbf{x}}-{{\textbf{z}}} |d\pi\\
 & + \pi_{\textbf{x}}(\Omega)+\pi_{{\textbf{z}}}(\Omega)-1
	\end{split}
\end{align}
Where $\Pi^p_{\lambda}(P_+, P_-)$ is the set consisting of positive measures $\pi\in \mathcal{M}_+(\Omega\times \Omega)$ which  are absolutely continuous with respect to the joint measure $dP_+\times dP_-$ and $\frac{d\pi_{\textbf{x}}}{dP_+}\in [p, p(1+\lambda)]$, $\frac{d\pi_{{\textbf{z}}}}{dP_-}\in [1-p, (1-p)(1+\lambda)] $.
%\footnote {{\color{red} (Franck) $[p, p(1+\lambda)]$ et $[1-p, (1-p)(1+\lambda)]$ me paraitrait plus clair}}
\end{Theorem}
%When the class are balanced, the constraints on $\pi$ became $\frac{d\pi_{\textbf{x}}}{d\mu}\in [\frac{1}{2}, \frac{1}{2}+\frac{1}{2}\lambda]$, $\frac{d\pi_{{\textbf{z}}}}{d\nu}\in [\frac{1}{2}, \frac{1}{2}+\frac{1}{2}\lambda] $ \footnote {{\color{red} (Franck) utile? obvious}}


\subsection{Classification and geometrical properties}
\label{sec:khr_properties}

\begin{figure*}
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=0.8\linewidth]{img/wass_reg_2moons_dist.png}
  \caption{Distribution of $\hat{f}$ conditionally to the classes.}
  \label{wass_pen:sub1}
\end{subfigure}%
\begin{subfigure}{.36\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/wass_reg_2moons_class.png}
  \caption{Level map of $\hat{f}$}
  \label{wass_pen:sub2}
\end{subfigure}
\caption{Hinge regularized Kantorovich-Rubinstein (hinge-KR) classification on the two moons problem}
\label{fig:wass_pen}
\end{figure*}
We note $\hat{f}$ the solution obtained by minimizing $\mathcal{L}^{hKR}_\lambda$ on a set of labeled examples and $f^*$ the solution of Eq.~\eqref{eq:reg_OT}. We don't assume that the solution found is optimal (i.e. $\hat{f}\neq f^*$) but we assume that $\hat{f}$ is 1-Lipschitz. Given a function $f$, a classifier based on $sign(f)$ and an example $x$, an adversarial example is defined as follows:
\begin{equation}
    adv(f,\textbf{x})=\underset{\textbf{z}\in \Omega | sign(f(\textbf{z}))=-sign(f(\textbf{x}))}{argmin}\parallel \textbf{x}-\textbf{z}\parallel.
\end{equation}
According to the 1-Lipschitz property of $\hat{f}$ we have 
\begin{equation}
\label{lowerbound}
%\parallel x- adv(\hat{f},x) \parallel \geq |\hat{f}(x)|.
|\hat{f}(\textbf{x})| \leq |\hat{f}(\textbf{x})-\hat{f}(adv(\hat{f},\textbf{x}))| \leq \parallel \textbf{x}- adv(\hat{f},\textbf{x}) \parallel.
\end{equation}
So $|\hat{f}(\textbf{x})|$ is a lower bound of the distance of $x$ to the separating boundary defined by $\hat{f}$ and thus a lower bound to the robustness to $l_2$ adversarial attacks. Thus, by minimizing $\mathbb{E} \left((1-\textbf{y}f(\textbf{x}))_+\right)$, we maximize the accuracy of the classifier and by maximizing the discrepancy of the image of $P_+$ and $P_-$ with respect to $f$ we maximize the robustness with respect to adversarial attack. The proposition below establishes that the gradient of the optimal function with respect to Eq.~\eqref{eq:reg_OT} has norm 1 almost surely, as for the unregularized case (Eq.~\eqref{eq:nabla_1}).
\begin{Proposition}\label{coro_norm1}
Let $\pi$ be the optimal measure of the dual version \eqref{eq:dual} of the hinge regularized optimal transport problem. Suppose that it is absolutely continuous with respect to Lebesgue measure. Then there exists at least a solution $f^*$ of \eqref{eq:dual} such that $||\nabla f^*||=1$ almost surely.
\end{Proposition}
 %Even we haven't prove it formally yet, empirical results suggest that given $\textbf{x}$, the image $tr_{f^*}(\textbf{x})$ of $\textbf{x}$ with respect to the transportation plan and $adv(\textbf{x})$ are in the same direction with respect to $x$ and this direction is $-f^*(\textbf{x})*\nabla_x f^*(\textbf{x})$ (i.e $adv(\textbf{x})\approx x-c_x*f^*(\textbf{x})*\nabla_x f^*(\textbf{x})$ and $tr_{f^*}(\textbf{x})\approx x-c'_x*f^*(\textbf{x})*\nabla_x f^*(\textbf{x})$ with $0 \leq c_x \leq c_x' \in \mathbb{R} $). This would link the adversarial attack to the optimal transport.
Furthermore, empirical results suggest that given $\textbf{x}$, the image $tr_{f^*}(\textbf{x})$ of $\textbf{x}$ by transport plan and $adv(\textbf{x})$ are in the same direction with respect to $\textbf{x}$ and the direction is % and 
 $-\nabla_x f^*(\textbf{x})$. Combining this direction with the Eq.~\eqref{lowerbound}, we will show empirically (sect.~\ref{sec:experimentation}) that  $$adv(\textbf{x})\approx x-c_x*f^*(\textbf{x})*\nabla_x f^*(\textbf{x})$$ and $$tr_{f^*}(\textbf{x})\approx x-c'_x*f^*(\textbf{x})*\nabla_x f^*(\textbf{x})$$ with $1 \leq c_x \leq c_x' \in \mathbb{R} $. It turns out that this corresponds to the definition of FGSM attacks \cite{Goodfellow2014a}. This suggests that in our frameworks, adversarial attacks amount to travel along the transportation path from the example to its transportation image.
 
The next proposition shows that, if the classes are well separated, maximizing the hinge-KR loss leads to a perfect classifier.% with no error.
\begin{Proposition}[Separable classes]\label{coro:epsilon}
Set  $P_+, P_-\in \mathcal{P}(\Omega)$ such that $P(Y=+1)=P(Y=-1)$ and $\lambda\geq 0$ and suppose that there exists $\epsilon>0$ such that
\begin{align}\label{coro:hipotesis}
	| {\textbf{x}}-{\textbf{{{\textbf{z}}}}} |> 2 \epsilon \ \ dP_+\times dP_- \text{ almost surely}
\end{align}
Then for each
\begin{align*}
	f_{\lambda}\in {\arg\sup}_{f\in \text{Lip}_{1/\epsilon}(\Omega)}\int_{\Omega}f(dP_+-dP_-)-\\
	\lambda \left( \int_{\Omega}(1-f)_+dP_+ +\int_{\Omega}(1+f)_+dP_-\right),
\end{align*}
it is satisfied that $L_1(f_{\lambda})=0.$ Furthermore if $\epsilon\geq 1$ then $f_{\lambda}$ is an optimal transport potential from $P_+$ to $P_-$ for the cost $| {\textbf{x}}-{{\textbf{z}}}|$.
\end{Proposition}
We show in Fig.~\ref{fig:wass_pen}, on the two moons problem, that in contrast to the vanilla classifier based on Wasserstein (Eq.~\eqref{eq:wass_vanilla_classif}), the proposed approach enables non overlapping distributions of $\hat{f}$ conditionally to the classes (Fig.~\ref{wass_pen:sub1}).
%Figure~\ref{fig:wass_pen} illustrates the approach on the two moons problem. Contrarily to the example with Wasserstein, we observe that the distributions of $f$ conditionally to the classes doesn't overlap (Figure~\ref{wass_pen:sub1}). 
In the same way, the 0-level cut of $\hat{f}$ (Fig.~\ref{wass_pen:sub2}) is a nearly optimal classification boundary. Moreover, the level cut of $\hat{f}$, on the support of the distributions, is close to the distance to this classification boundary.
%, corresponds approximately to the distance to the classification boundary.  

==> cvpr_parts/lipschitz_section.tex <==
\subsection{1-Lipschitz gradient norm preserving network}
In order to build a deep learning classifier based on the hinge-KR optimization problem (Eq.~\eqref{eq:reg_OT}), we have to constrain the Lipschitz constant of the neural network to be equal to 1.  It is known that evaluating it exactly is a NP-hard problem~\cite{NIPS2018_7640}. The simplest way to constraint a network to be 1-Lipschitz is to impose this 1-Lipschitz property to each layer. For dense layers, the initial version of WGAN \cite{Arjovsky2017} consisted of clipping the weights of the layers. However, this is a very crude way to upper-bound Lipschitz constant. Normalizing by the Frobenius norm has also been proposed in~\cite{SalimansK16}. In this paper, we use spectral normalization as proposed in~\cite{Miyato2018SpectralNF}, since the spectral norm is equals to the Lipschitz constant of the layer. At the inference step, we normalize the weights of each layer by the spectral norm of the matrix. This spectral norm is computed by iteratively evaluating the largest singular value with the power iteration algorithm~\cite{GOLUB200035}. This is done during the forward step and taken into account for the gradient computation. In the case of 2D-convolutional layers, normalizing by the spectral norm of convolution kernels is not enough and a supplementary multiplicative constant $\Lambda$ is required (the regularization is then done by dividing $W$ by $\Lambda||W||$). We propose, for zero padding, a tighter estimation of $\Lambda$ than the one proposed in~\cite{cisse_parseval_2017}, computing the average duplication factor of non zero padded values in the feature map:

\begin{equation}
\Lambda=\sqrt{\frac{(k.w-\bar{k}.(\bar{k}+1)).(k.h-\bar{k}.(\bar{k}+1))}{h.w}}
\label{eq:ConvApproxLip}
\end{equation}
for a kernel size equals to $k=2*\bar{k}+1$.
Even if this constant doesn't provide a strict upper bound of the Lipschitz constant (for instance, when the higher values are located in the center of the picture), it behaves very well empirically.
Convolution with stride, pooling layers, detailed explanations and demonstrations are discussed in Appendix~\ref{sec:convStride}.\\

As shown in Property~\ref{coro_norm1}, the optimal function $f^*$ with respect to Eq.~\eqref{eq:reg_OT}, verifies $||\nabla f^* ||=1$ almost surely (\textit{gradient norm preserving} (GNP) architecture~\cite{pmlr-v97-anil19a} ). We apply the approach described in~\cite{pmlr-v97-anil19a}, based on the use of specific activation functions and a process of normalization  of the weights. Two norm preserving activation functions are proposed: i)\ \textbf{GroupSort2} : sorting the vector by pairs, ii) \textbf{FullSort} : sorting the full vector.
These functions are vector-wise rather than element-wise. We also use the P-norm pooling~\cite{boureau2010}, with $P=2$ which is a norm-preserving average pooling.
Concerning linear functions, a weight matrix $W$ is gradient norm preserving if and only if all the singular values of $W$ are equals to $1$. In \cite{pmlr-v97-anil19a}, the authors propose to use the Björck orthonormalization algorithm \cite{bjorck71Ortho}. This algorithm is fully differential and, as for spectral normalization, is applied during the forward inference, and taken into account for back-propagation (see Appendix~\ref{app:normpreserving} for details). We don't consider BCOP \cite{qian_l2-nonexpansive_2019}, which performs slightly better that Björck for convolution but at an higher computation cost. We developed a full tensorflow~\cite{tensorflow2015-whitepaper} implementation in an opensource library, called \Deellip, that enables training of $k$-Lipschitz neural networks, and exporting them as standard layers for inference. 
\subsection{Multi-class hinge-KR classifier}
To adapt our approach to the multi-class case, we propose to use $q$ binary one-vs-all classifiers, where $q$ is the number of classes. The set of labels is now $Y=\{C_1,\ldots,C_q\}$. We name $P_k=\mathbb{P}(X|Y= C_k)$ and $\neg P_k=\mathbb{P}(X|Y\not = C_k)$ the  conditional  distributions  with  respect  to  $Y$. We obtain the following optimization problem :
\begin{equation}
\label{eq:hkr_multi}
\begin{split}
&\underset{f_1,\ldots,f_q \in Lip_1(\Omega)}{\text{sup}}-\mathcal{L}^{hKR}_\lambda(f_1,\ldots,f_q) \\
&\text{where}\\
&\mathcal{L}^{hKR}_\lambda(f_1,\ldots,f_q) = \sum_{k=1}^q \left[\underset{\textbf{x}  \sim \neg P_k}{\mathbb{E}} \left[f_k(\textbf{x})\right] -\underset{\textbf{x} \sim P_k}{\mathbb{E}}\left[f_k(\textbf{x})\right] \right.\\ 
 & \left. \quad \quad \quad \quad \quad +\lambda\underset{\textbf{x}}{\mathbb{E}} \left(m-(2*\underset{y=C_k}{\mathbbm{1}} -1).f_k(x)  \right)_+ \right].
\end{split}
\end{equation}
The global architecture is the same as the binary one except that the last layer has $q$ outputs. For this last layer, each weights corresponding to each output neuron are normalized independently creating $q$ 1-Lipschitz functions with gradient norm preserving properties. With this architecture, the optimal transport interpretation is still valid. The class predicted corresponds to the argmax of the classifier functions. With this approach, the provable robustness lower-bound is the half of the difference between the max and the second max values of $\{f_1(x),\ldots,f_q(x)\}$.  

In \cite{li2019preventing}, Li et al. use classical multi-class hinge loss based on un-centered margin and apply constraint on the entire last layers rather than doing it independently. It allows to a lower provable adversarial robustness bound than ours. However, the $f_1,\ldots,f_q$ obtain in this setting are no more 1-Lipschitz one by one, making the adversarial robustness bounds not comparable directly (see Appendix~\ref{sec:robustness_bounds}).

==> cvpr_parts/wass_distance_cvpr.tex <==
In this paper we only consider the Wasserstein-1 distance, also called Earth-mover, and noted $\W$ for $\W_1$.
The $1$-Wasserstein distance between two probability distributions $\mu$ and $\nu$ in $\Omega$, and its dual formulation by Kantorovich-Rubinstein duality \cite{villani2008}, is defined as the solution of:
\begin{subequations}

\begin{align}
\W(\mu,\nu) & = \inf_{\pi \in \Pi(\mu,\nu)}\underset{x,z \sim \pi}{\mathbb{E}}\parallel \textbf{x}-\textbf{z} \parallel \label{wasserstein}\\
  & =\sup_{f \in Lip_1(\Omega)} \underset{\textbf{x} \sim \mu}{\mathbb{E}} \left[f(\textbf{x} )\right] -\underset{\textbf{x}  \sim \nu}{\mathbb{E}} \left[f(\textbf{x} )\right] \label{kantorovich}
\end{align}
\end{subequations}

where $\Pi(\mu,\nu)$ is the set of all probability measures on $\Omega\times \Omega$ with marginals $\mu$ and $\nu$ and $Lip_1(\Omega)$ denotes the space of 1-Lipschitz functions over $\Omega$. 
Although, the infimum in Eq.~\eqref{wasserstein} is not tractable in general, the dual problem can be estimated through the optimization of a regularized neural network. This approach has been introduced in WGAN  \cite{Arjovsky2017} where $Lip_1(\Omega)$ is approximated by the set of neural networks with bounded weights (better approximations of $Lip_1(\Omega)$ will be discussed in Section~\ref{sec:lip_const}). 

We consider a binary classification problem on feature vector space $X\subset \Omega$ and and labels $Y= \{-1,1\}$. We name $P_+=\mathbb{P}(X|Y=1)$ and  $P_-=\mathbb{P}(X|Y=-1)$, the conditional distributions with respect to Y. We note $p=P(Y=1)$ and $1-p=P(Y=-1)$ the apriori class distribution. The classification problem is balanced when $p=\frac{1}{2}$.\\

In WGAN, \cite{Arjovsky2017} proposed to use the learned neural network (denoted $\hat{f}$ in the following),  by maximizing the Eq.~\eqref{kantorovich}, as a discriminator between fake and real images, in analogy with GAN~\cite{Goodfellow2014}.
%\footnote{{\color{red} (FRANCK:proposition de reformulation, l'ancienne version est commentee)}} 
%In analogy with GAN~\cite{Goodfellow2014}, the function obtained by optimizing equation~\ref{kantorovich} (denoted $\hat{f}$ in the following) in WGAN behaves like a discriminator between fake and real examples. 
To build a classifier based on $\hat{f}$, one can simply note that if  $f^*$ is an optimal solution of Eq.~\eqref{kantorovich}, then  $f^* + C, C\in \mathbb{R}$, is also optimal. Centering the function $f^*$ (resp. $\hat{f}$), Eq.~\eqref{eq:wass_vanilla_classif}, enables classification according to the sign of $f_c^*(x)$ (resp.$\hat{f_c}$ for the empirical solution).
%\footnote{{\color{red} (FRANCK:idem, l'ancienne version est commentee)}} 
%Let $f^*$ is an optimal solution of Equation~\eqref{kantorovich}, then $f^* + c, c\in \mathbb{R}$, is also optimal. In order to build a classifier, the simplest solution consists in centering the function $f^*$ (resp. $\hat{f}$)  as follows:The class correspond to the sign of $f_c^*(x)$ (resp.$\hat{f_c}$ for the empirical solution). 
\begin{equation}
\label{eq:wass_vanilla_classif}
f_c^*(\textbf{x} )=f^*(\textbf{x} )-\frac{1}{2}\left(\underset{\textbf{z}  \sim P_+}{\mathbb{E}} \left[f^*(\textbf{z} )\right] +\underset{\textbf{z}  \sim P_-}{\mathbb{E}} \left[f^*(\textbf{z} )\right]\right).
\end{equation}

Such a classifier would exhibit good properties in terms of robustness for two main reasons: First, it has been shown in \cite{villani2008} that the function $f^*$ is directly related to the cost of transportation between two points linked by the transportation plan %(when $\pi^*(x=y)=0$) 
as follows:

%Let denote $\hat{f}$ the function obtained by optimizing equation~\ref{kantorovich} 
%In the balanced discrete case, it has been shown {\color{red} (FRANCK: Ref ?)} that the optimal transport plan is an 1-1 transportation plan (i.e. $\Pi^*_{i,j} \in\{0,1\}$) and:
%\begin{equation}
%\forall i,j\text{ s.a. }\Pi^*_{i,j}=1,  F^*_i-F^*_{n+j}= C_{i,j}
%\end{equation}
%where $F^*$ is the optimal solution of the dual optimal transport problem. 

\begin{equation}
\label{eq:transport_cost}
\mathbb{P}_{\textbf{x},\textbf{z}\sim \pi^*}(f^*(\textbf{x})-f^*(\textbf{z})=||\textbf{x}-\textbf{z}||)=1.
\end{equation}
 %This shows that the function $f^*$ is directly related to the cost of transportation between two point linked by the transportation plan. 
 Second, it was shown in \cite{gulrajani2017improved,pmlr-v97-anil19a}, that this optimal solution also induces a property stronger  than 1-Lipschitz:
\begin{equation}
\label{eq:nabla_1}
||\nabla f^* ||=1 \text{ almost surely on the support of }\pi^*.
\end{equation}
%The previous properties with respect to the transportation plan and the 1-Lipschitz constraint also underlined good properties in terms of robustness. 

However, applying this vanilla classifier (Eq.~\eqref{eq:wass_vanilla_classif}) to a toy dataset such as the two-moons problem, leads to a poor accuracy.
Indeed, Figures~\ref{wass:sub1} and~\ref{wass:sub2} present respectively the distribution of the values of $\hat{f_c}(x)$ conditionally to the classes and the level map of $\hat{f_c}$. We can observe that, even if the classes are easily separable, the distributions of the values of $\hat{f_c}$ conditionally to the class overlap. Thus, the 0-level threshold on $\hat{f_c}$ does not correspond to the optimal separator (even if it is better than random). Intuitively, $\hat{f_c}$  
%{\color{red} (FRANCK: $f*$?)} 
maximizes the difference of the expectancy of the image of  
the two distributions but do not try to minimize their overlap (Fig.~\ref{wass:sub1}). 
%We can also note %remark 
%that, for $\W$ 
%and the Earth-mover distance, 
%the solution is not unique.
%{\color{red} ( Thibaut ) on fait une analogie avec les WGAN avant de d'expliciter comment on fait la classification a partir de  f ( eq 11 ), ce qui risque plus d'embrouiller le lecteur. ( Entre le discriminateur d'un GAN, la régularization de Wasserstein d'un GAN et notre classifier, la confusion peut vite arriver )\\
%MAthieu -> exact!}\\
%{FRANCK -> yes tentative d'explicitation differente dans l'intro! plus qqes reofrmulations ci dessous}
%In analogy with GAN \cite{Goodfellow2014}, the network that computes the function $f$ with respect to Kantorovich-Rubinstein formulation in WGAN can be viewed as a classifier.  
%{\color{red}(MATHIEU) : faire l'exemple avec le transport optimal et le seuil)}

\begin{figure*}
\centering
\begin{subfigure}{.4\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/wass_2moons_dist.png}
  \caption{Distribution of $\hat{f_c}$ conditionally to the classes}
  \label{wass:sub1}
\end{subfigure}%
\begin{subfigure}{.36\textwidth}
  \centering
  \includegraphics[width=1\linewidth]{img/wass_2moons_class.png}
  \caption{Level map of $\hat{f_c}$}
  \label{wass:sub2}
\end{subfigure}
\caption{Wasserstein classification (Eq.~\eqref{eq:wass_vanilla_classif}) on the two moons.}
\label{fig:wass}
\end{figure*}

